On Semi-supervised Estimation of Discrete Distributions under f-divergences

We study the problem of estimating the joint probability mass function (pmf) over two random variables. In particular, the estimation is based on the observation of $m$ samples containing both variables and $n$ samples missing one fixed variable. We adopt the minimax framework with $l^p_p$ loss functions. Recent work established that univariate minimax estimator combinations achieve minimax risk with the optimal first-order constant for $p \ge 2$ in the regime $m = o(n)$, questions remained for $p \le 2$ and various $f$-divergences. In our study, we affirm that these composite estimators are indeed minimax optimal for $l^p_p$ loss functions, specifically for the range $1 \le p \le 2$, including the critical $l_1$ loss. Additionally, we ascertain their optimality for a suite of $f$-divergences, such as KL, $\chi^2$, Squared Hellinger, and Le Cam divergences.

==> course_header.tex <==
%\pagestyle{myheadings}
%\markright{P. Golland and G. W. Wornell}
\newcommand{\thecoursename}{
Massachusetts Institute of Technology \\
Department of Electrical Engineering and Computer Science

\textsc{6.437 Inference and Information}
}

\newcommand{\theterm}{Spring 2016}
\thispagestyle{empty}



==> defs.tex <==
\newcommand{\courseheader}{
\vspace*{-1in}
\begin{center}
\thecoursename \\
\theterm
\vspace*{0.1in}
\hrule
\end{center}
}

\newcounter{psctr}
\newcounter{probctr}[psctr]
%\renewcommand{\theprobctr}{\arabic{psctr}.\arabic{probctr}}
\newcommand{\problem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr}\nopagebreak

\noindent{#1}

}
\newcommand{\extraproblem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr\ (practice)}\nopagebreak

\noindent{#1}

}

\newcommand{\putfig}[3]{%
\centering
\includegraphics[width=#2]{#1}
\caption{#3}
}

\newcommand{\putfigtwo}[4]{%
\centering
\subfloat[\ ]{\includegraphics[width=#3]{#1}}\\ \vspace*{3ex}
\subfloat[\ ]{\includegraphics[width=#3]{#2}}
\caption{#4}
}

\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif
\DeclareMathAlphabet{\mathbbb}{U}{bbold}{m}{n}  % bb bold numbers
% can also use bbm package, which seems to work w/o pdflatex

%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbb}{bbold}


% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}  
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}

\newcommand{\fxfm}{\stackrel{\mathcal{F}}{\longleftrightarrow}}
\newcommand{\lxfm}{\stackrel{\mathcal{L}}{\longleftrightarrow}}
\newcommand{\zxfm}{\stackrel{\mathcal{Z}}{\longleftrightarrow}}

\DeclareMathOperator*{\gltop}{\gtreqless}
\newcommand{\glt}{\;\gltop^{\Hh=\svH_1}_{\Hh=\svH_0}\;}
\newcommand{\glty}{\;\gltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\gltby}{\;\gltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\DeclareMathOperator*{\geltop}{\genfrac{}{}{0pt}{}{\ge}{<}}
\newcommand{\gelty}{\;\geltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\geltby}{\;\geltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
%\renewcommand{\pe}{\Prob{e}}
\renewcommand{\defeq}{\triangleq}
\newcommand{\like}{\svlike}
\newcommand{\rvlike}{\mathssf{L}}
\newcommand{\sst}{\cl}
\newcommand{\svlike}{L}
\newcommand{\llike}{\rvllike}
\newcommand{\rvllike}{\cl}
\newcommand{\svllike}{l}
\newcommand{\lliket}{\tel}
\newcommand{\bllike}{\rvbllike}
\newcommand{\rvbllike}{\boldsymbol{\cl}}
\newcommand{\svbllike}{\mathbf{l}}
\newcommand{\Qb}{\overline{Q}}
\renewcommand{\comb}[2]{\binom{#1}{#2}}


%% Random/sample variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
% Capitals
\newcommand{\rvA}{{\mathssf{A}}}	% A
\newcommand{\svA}{A}
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\svbA}{{\mathbf{A}}}
\newcommand{\rvFh}{{\hat{\mathssf{F}}}}	% F
\newcommand{\rvF}{{\mathssf{F}}}
\newcommand{\rvHh}{{\hat{\mathssf{H}}}}	% H
\newcommand{\rvH}{{\mathssf{H}}}
\newcommand{\svH}{H}
\newcommand{\svHh}{{\hat{\svH}}}
\newcommand{\rvL}{{\mathssf{L}}}	% L
\newcommand{\svL}{L}
\newcommand{\rvN}{{\mathssf{N}}}	% N
\newcommand{\rvR}{{\mathssf{R}}}	% R
\newcommand{\rvRh}{{\hat{\rvR}}}
\newcommand{\rvS}{{\mathssf{S}}}	% S
\newcommand{\rvSh}{{\hat{\rvS}}}
\newcommand{\rvW}{{\mathssf{W}}}	% W
\newcommand{\rvX}{{\mathssf{X}}}  	% X, random variable
\newcommand{\svX}{X}		  	
\newcommand{\rvXt}{{\tilde{\rvX}}}
\newcommand{\rvY}{{\mathssf{Y}}}	% Y

\newcommand{\rvZ}{{\mathssf{Z}}}	% Z
\newcommand{\rvbZ}{{\mathbsf{Z}}}	
\newcommand{\svZ}{{{Z}}}	
\newcommand{\svbZ}{{\mathbf{Z}}}	

\newcommand{\rva}{{\mathssf{a}}}	% a
\newcommand{\rvah}{{\hat{\rva}}}
\newcommand{\sva}{a}
\newcommand{\svah}{{\hat{\sva}}}
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\svba}{{\mathbf{a}}}
%
\newcommand{\rvb}{{\mathssf{b}}}	% b
\newcommand{\rvbh}{{\hat{\rvb}}}
\newcommand{\svb}{b}
\newcommand{\svbh}{{\hat{\svb}}}
\newcommand{\rvbb}{{\mathbsf{b}}}
\newcommand{\svbb}{{\mathbf{b}}}
%
\newcommand{\rvc}{{\mathssf{c}}}	% c
\newcommand{\rvch}{{\hat{\rvc}}}
\newcommand{\svc}{c}
\newcommand{\svch}{{\hat{\svc}}}
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\svbc}{{\mathbf{c}}}
%
\newcommand{\rvbd}{{\mathbsf{d}}}	% d
\newcommand{\rve}{{\mathssf{e}}}	% e
\newcommand{\sve}{e}
\newcommand{\rvbfe}{{\mathbsf{e}}}
\newcommand{\svbfe}{{\mathbf{e}}}
\newcommand{\rvf}{{\mathssf{f}}}	% f
\newcommand{\svf}{f}
\newcommand{\rvbff}{{\mathbsf{f}}}
\newcommand{\svbff}{{\mathbf{f}}}
\newcommand{\rvg}{{\mathssf{g}}}	% h
\newcommand{\svg}{g}
\newcommand{\rvh}{{\mathssf{h}}}	% h
\newcommand{\rvk}{{\mathssf{k}}}	% k
\newcommand{\svk}{k}
\newcommand{\rvm}{{\mathssf{m}}}	% m
\newcommand{\rvbm}{{\mathbsf{m}}}  
\newcommand{\svm}{{{m}}}
\newcommand{\svbm}{{\mathbf{m}}}
\newcommand{\rvn}{{\mathssf{n}}}	% n
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\rvq}{{\mathssf{q}}}	% q
\newcommand{\svq}{q}
\newcommand{\rvr}{{\mathssf{r}}}	% r
\newcommand{\rvbr}{{\mathbsf{r}}}
\newcommand{\svr}{{r}}
\newcommand{\svbr}{{\mathbf{r}}}
\newcommand{\rvs}{{\mathssf{s}}}	% s
\newcommand{\svs}{s}
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\svbs}{{\mathbf{s}}}
\newcommand{\rvt}{{\mathssf{t}}}	% t
\newcommand{\svt}{t}
\newcommand{\rvbt}{{\mathbsf{t}}}
\newcommand{\svbt}{{\mathbf{t}}}
\newcommand{\rvu}{{\mathssf{u}}}	% u
\newcommand{\svu}{u}
\newcommand{\svuh}{{\hat{\svu}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvv}{{\mathssf{v}}}	% v
\newcommand{\svv}{v}
\newcommand{\svvh}{{\hat{\svv}}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvvh}{{\hat{\rvv}}}
\newcommand{\rvw}{{\mathssf{w}}}	% w
\newcommand{\svw}{w}
\newcommand{\rvwh}{{\hat{\rvw}}}
\newcommand{\svwh}{{\hat{\svw}}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvx}{{\mathssf{x}}}	% x, random variable
\newcommand{\rvxh}{{\hat{\rvx}}}
\newcommand{\rvxt}{{\tilde{\rvx}}}
\newcommand{\svx}{x}			% sample value
\newcommand{\svxh}{{\hat{\svx}}}
\newcommand{\svxt}{{\tilde{\svx}}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvbxh}{{\hat{\rvbx}}}
\newcommand{\rvbxt}{{\tilde{\rvbx}}}
\newcommand{\svbx}{{\mathbf{\svx}}}
\newcommand{\svbxt}{{\tilde{\svbx}}}
\newcommand{\svbxh}{{\hat{\mathbf{x}}}}
\newcommand{\rvy}{{\mathssf{y}}}	% y
\newcommand{\rvyh}{{\hat{\mathssf{y}}}}
\newcommand{\svy}{y}
\newcommand{\rvyt}{{\tilde{\rvy}}}
\newcommand{\svyt}{{\tilde{\svy}}}
\newcommand{\svyh}{{\hat{\svy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvbyt}{{\tilde{\rvby}}}
\newcommand{\svby}{{\mathbf{y}}}
\newcommand{\svbyt}{{\tilde{\svby}}}
\newcommand{\rvz}{{\mathssf{z}}}	% z
\newcommand{\rvzh}{{\hat{\rvz}}}
\newcommand{\rvzt}{{\tilde{\rvz}}}
\newcommand{\svz}{z}
\newcommand{\svzh}{{\hat{\svz}}}
\newcommand{\rvbz}{{\mathbsf{z}}}
\newcommand{\svbz}{{\mathbf{z}}}

% Handle uppercase Greek differently
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\svTh}{\Theta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\svbTh}{\boldsymbol{\Theta}}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\svPh}{\Phi}
\newcommand{\rvbPh}{\bsfPhi}
\newcommand{\svbPh}{\boldsymbol{\Phi}}

\newcommand{\ddx}{\frac{\diff}{\diff \svx}}
\newcommand{\ddbx}{\frac{\diff}{\diff\svbx}}
\newcommand{\ppx}{\frac{\p}{\p \svx}}
\newcommand{\ppbx}{\frac{\p}{\p\svbx}}
\newcommand{\ddy}{\frac{\diff}{\diff \svy}}
\newcommand{\ddby}{\frac{\diff}{\diff\svby}}
\newcommand{\ppy}{\frac{\p}{\p \svy}}
\newcommand{\ppby}{\frac{\p}{\p\svby}}

\def\setTh{\text{$\mksetTh$}}  % make caligraphic Theta
\def\mksetTh{\setbox0\hbox{$\mathcal{O}$}%
    \rlap{\hbox to \wd0{\hss\raisebox{.2ex}{\hspace*{.07em}\textbf{-}}\hss}}\box0}

%  --add new macros below this line--

\newcommand\indep{\protect\mathpalette{\protect\indepT}{\perp}}
\def\indepT#1#2{\mathrel{\rlap{$#1#2$}\mkern3mu{#1#2}}}
\newcommand{\truex}{\svx}
\newcommand{\obsy}{\svy}
\newcommand{\dummyx}{a}
\newcommand{\dummybx}{\ba}
\newcommand{\dummyy}{b}
\newcommand{\dummyby}{\bb}
\newcommand{\dummyz}{c}
\newcommand{\Db}{D_\mathrm{B}}   % binary divergence
\newcommand{\Hb}{H_\mathrm{B}}   % binary entropy
\newcommand{\Hhb}{\Hh_\mathrm{B}} % Bayes decision rule
\newcommand{\Hhnp}{\Hh_\mathrm{NP}} % Neyman-Pearson decision rule
\newcommand{\Hhm}{\Hh_\mathrm{M}} % minimax decision rule
\newcommand{\alphA}{\cA}
\newcommand{\alphB}{\cB}
\newcommand{\alphE}{\cE}
\newcommand{\alphL}{\cL}
\newcommand{\alphV}{\cV}
\newcommand{\cardV}{M}
\newcommand{\alphR}{\cR}
\newcommand{\alphS}{\cS}
\newcommand{\alphT}{\cT}
\newcommand{\alphU}{\cU}
\newcommand{\alphW}{\cW}
\newcommand{\alphX}{\cX}
\newcommand{\cardX}{L}
\newcommand{\alphY}{\cY}
\newcommand{\alphZ}{\cZ}
\newcommand{\cardY}{M}
\newcommand{\efdim}{K}
\newcommand{\dimX}{K}
\newcommand{\dimY}{N}
\newcommand{\alphH}{\cH}

\newcommand{\sumX}{\sum_{\svx\in\alphX}}
\newcommand{\sumY}{\sum_{\svy\in\alphY}}

\newcommand{\fisher}{J}
\newcommand{\Fisher}{\bJ}
\newcommand{\bfisher}{\bJ}
\newcommand{\score}{S}
\newcommand{\Score}{\bS}
\newcommand{\bscore}{\bS}
\newcommand{\objfn}{\varphi}
\newcommand{\varobjfn}{\tilde{\objfn}}




\renewcommand{\emptyset}{\varnothing}
\renewcommand{\approx}{\cong}

% functional dot

\def\fndot{\, \cdot \,}

% exponential

\newcommand{\eexp}[1]{e^{#1}}

% iid

\newcommand{\iid}{i.i.d.}

% convergence

\newcommand{\convp}{\stackrel{\mathrm{p}}{\longrightarrow}}
\newcommand{\convas}{\stackrel{\mathrm{a.s.}}{\longrightarrow}}
\newcommand{\convwpone}{\convas}
\newcommand{\convd}{\stackrel{\mathrm{d}}{\longrightarrow}}
\newcommand{\convD}{\stackrel{\mathrm{D}}{\longrightarrow}}

% stochastic approximation

\newcommand{\pun}{p_\circ}
\newcommand{\punh}{\hat{p}_\circ}
\newcommand{\qun}{q_\circ}
\newcommand{\qunh}{\hat{q}_\circ}

\newcommand{\genf}{f}
\newcommand{\genfb}{\bar{f}}
\newcommand{\genfbh}{\hat{\bar{\rvf}}}


\DeclareMathOperator{\neb}{ne}
\newcommand{\bep}{{\boldsymbol{\varepsilon}}}

\newcommand{\gauss}{\mathtt{N}}
\newcommand{\bern}{\mathtt{B}}
\newcommand{\unif}{\mathtt{U}}
\newcommand{\poiss}{\mathtt{P}}
\newcommand{\betad}{\mathtt{Beta}}
\newcommand{\gammad}{\mathtt{Gamma}}
\newcommand{\expd}{\mathtt{E}}
\newcommand{\expfam}{\mathcal{E}}

\newcommand{\kron}{\mathbbb{1}}
%\newcommand{\kron}{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}
%\DeclareMathOperator{\kron}{\leavevmode\hbox{\small\rm1\normalsize\kern-.33em1}}

\newcommand{\dotleq}{\stackrel{.}{\leq}}
\newcommand{\dotlt}{\stackrel{.}{<}}
\newcommand{\dotgeq}{\stackrel{.}{\geq}}
\newcommand{\dotgt}{\stackrel{.}{>}}
\newcommand{\Ps}[1]{P\left\{#1\right\}}
\newcommand{\Qs}[1]{Q\left\{#1\right\}}

\newcommand{\diff}{\mathrm{d}}

% from 6.008

\newcommand{\sd}{p_\rvx}  % steady-state distribution
\newcommand{\td}{W}    % transition distribution
\newcommand{\sdv}{\bp_\rvx}  % steady-state distribution vector
\newcommand{\tdm}{\bW}  % transition distribution matrix
\newcommand{\tde}{w}    % transition distribution matrix elements
\newcommand{\sde}{p}    % steady-state distribution vector elements
\newcommand{\bigO}{\mathcal{O}}



==> gww_chars.tex <==
% ABBREVIATIONS FOR CHARACTERS IN VARIOUS FONTS
% Edited by Polina Golland -- Jan 14, 2007

% STANDARD CHARACTERS

\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bah}{{\hat{\ba}}}
\newcommand{\ah}{{\hat{a}}}
\newcommand{\Ah}{{\hat{A}}}
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\at}{{\tilde{a}}}
\newcommand{\bat}{{\tilde{\ba}}}
\newcommand{\At}{{\tilde{A}}}
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\ac}{a^{\ast}}

\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bbt}{{\tilde{\bb}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\tb}{{\tilde{b}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\hb}{{\hat{b}}}
\newcommand{\hB}{{\hat{B}}}
\newcommand{\bB}{{\mathbf{B}}}

\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\bch}{{\hat{\mathbf{c}}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\ct}{{\tilde{c}}}
\newcommand{\Ct}{{\tilde{C}}}
\newcommand{\ctc}{\ct^{\ast}}

\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\hd}{{\hat{d}}}  % old: \dh
\newcommand{\dt}{{\tilde{d}}}
\newcommand{\bdt}{{\tilde{\bd}}}
\newcommand{\Dt}{{\tilde{D}}}
\newcommand{\dtc}{\dt^{\ast}}

\newcommand{\et}{{\tilde{e}}}
\newcommand{\bfe}{{\mathbf{e}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cEt}{{\tilde{\cE}}}
\newcommand{\cEb}{{\bar{\cE}}}
\newcommand{\bcE}{{\mathbf{\cE}}}  % bf cal E doesn't exist

\newcommand{\bff}{{{\mathbf{f}}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\ft}{{\tilde{f}}}
\newcommand{\Ft}{{\tilde{F}}}
\newcommand{\Fh}{{\hat{F}}}
\newcommand{\ftc}{\ft^{\ast}}
\newcommand{\bft}{{\tilde{\bff}}}
\newcommand{\bFt}{{\tilde{\bF}}}
\newcommand{\fh}{{\hat{f}}}

\newcommand{\bg}{{\mathbf{g}}}
\newcommand{\gt}{{\tilde{g}}}
\newcommand{\bgt}{{\tilde{\bg}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\Gt}{{\tilde{\bG}}}

\newcommand{\hti}{{\tilde{h}}}
\newcommand{\Hti}{{\tilde{H}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bht}{{\tilde{\bh}}}
\newcommand{\Hh}{{\hat{H}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bHh}{{\hat{\mathbf{H}}}}
\newcommand{\cH}{\mathcal{H}}

\newcommand{\ih}{{\hat{\imath}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\It}{{\tilde{I}}}

\newcommand{\jh}{{\hat{\jmath}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\Jt}{{\tilde{J}}}

\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\Kt}{{\tilde{K}}}
\newcommand{\Kh}{{\hat{K}}}
\newcommand{\cK}{{\mathcal{K}}}

\newcommand{\tl}{\tilde{l}}
\newcommand{\tel}{\tilde{\cl}}
\newcommand{\cl}{\ell}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\cL}{{\mathcal{L}}}

\newcommand{\mb}{{\mathbf{m}}}
\newcommand{\mh}{{\hat{m}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\cM}{{\mathcal{M}}}


\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\Nt}{{\tilde{N}}}
\newcommand{\tN}{{\tilde{N}}}  % backward compatibility

\newcommand{\bo}{{\mathbf{o}}}
\newcommand{\cO}{{\mathcal{O}}}

\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cPh}{{\hat{\mathcal{P}}}}
\newcommand{\ph}{{\hat{p}}}
\newcommand{\Ph}{{\hat{P}}}
\newcommand{\pt}{{\tilde{p}}}

\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\qt}{{\tilde{q}}}

\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\Rt}{{\tilde{R}}}

\newcommand{\sh}{{\hat{s}}}
\newcommand{\sck}{{\check{s}}}
\newcommand{\shh}{{\Hat{\Hat{s}}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bsh}{{\hat{\mathbf{s}}}}
\newcommand{\bsc}{{\check{\mathbf{s}}}}
\newcommand{\bshh}{{\Hat{\Hat{\mathbf{s}}}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\st}{{\tilde{s}}}

\newcommand{\tilt}{{\tilde{t}}} % To avoid conflict with \tt
\newcommand{\boldt}{{\mathbf{t}}} % To avoid conflict with beta
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\cT}{{\mathcal{T}}}

\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bUt}{{\tilde{\bU}}}
\newcommand{\ut}{{\tilde{u}}}
\newcommand{\cU}{{\mathcal{U}}}

\newcommand{\vh}{{\hat{v}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\cV}{{\mathcal{V}}}

\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\cW}{{\mathcal{W}}}

\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\bxt}{{\tilde{\bx}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\Xt}{{\tilde{X}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\bXt}{{\tilde{\bX}}}
\newcommand{\xh}{{\hat{x}}}
\newcommand{\xc}{{\check{x}}}
\newcommand{\xhh}{{\Hat{\Hat{x}}}}
\newcommand{\bxh}{{\hat{\bx}}}
\newcommand{\bxc}{{\check{\bx}}}
\newcommand{\bxhh}{{\Hat{\hat{\bx}}}}

\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\byt}{{\tilde{\by}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\Yt}{{\tilde{Y}}}
\newcommand{\yt}{{\tilde{y}}}
\newcommand{\yh}{{\hat{y}}}

\newcommand{\zt}{{\tilde{z}}}
\newcommand{\zh}{{\hat{z}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cZ}{{\mathcal{Z}}}



% GREEK CHARACTERS

\newcommand{\al}{\alpha}
\newcommand{\bal}{{\boldsymbol{\al}}}
\newcommand{\balh}{{\hat{\boldsymbol{\al}}}}
\newcommand{\alh}{{\hat{\al}}}

\newcommand{\bt}{\beta}
\newcommand{\bbeta}{{\boldsymbol{\bt}}}
\newcommand{\btt}{{\tilde{\bt}}}
\newcommand{\btht}{{\hat{\bt}}}

\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\bGa}{{\boldsymbol{\Gamma}}}
\newcommand{\gh}{{\hat{\g}}}

\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\Deh}{{\hat{\Delta}}}
\newcommand{\bde}{{\boldsymbol{\de}}}
\newcommand{\bDe}{{\boldsymbol{\De}}}

%\newcommand{\e}{\epsilon}
%\newcommand{\eps}{\varepsilon}
\newcommand{\eps}{\epsilon}

\newcommand{\etah}{{\hat{\eta}}}
\newcommand{\boldeta}{{\boldsymbol{\eta}}} % since \beta is aleady taken

\newcommand{\bpi}{{\boldsymbol{\pi}}}

\newcommand{\pht}{{\tilde{\phi}}}
\newcommand{\Pht}{{\tilde{\Phi}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bvphi}{{\boldsymbol{\varphi}}}


\newcommand{\bpsi}{{\boldsymbol{\psi}}}
\newcommand{\pst}{{\tilde{\psi}}}
\newcommand{\Pst}{{\tilde{\Psi}}}

\newcommand{\s}{\sigma}
\newcommand{\sih}{\hat{\sigma}}

\newcommand{\z}{\zeta}
\newcommand{\ztt}{{\tilde{\z}}}
\newcommand{\ztb}{{\bar{\z}}}

% \newcommand{\th}{\theta} % symbol name used by other latex package
\newcommand{\thh}{{\hat{\theta}}}
\newcommand{\Thh}{{\hat{\Theta}}}
\newcommand{\Th}{\Theta}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand{\bTh}{{\boldsymbol{\Theta}}}
\newcommand{\bThh}{{\hat{\bTh}}}
\newcommand{\Tht}{{\tilde{\Theta}}}

\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\lam}{\lambda}  % backward compatibility
\newcommand{\Lam}{\Lambda}  % backward compatibility
\newcommand{\bla}{{\boldsymbol{\la}}}
\newcommand{\bLa}{{\boldsymbol{\La}}}
\newcommand{\lah}{{\hat{\lam}}}



\newcommand{\bmu}{{\boldsymbol{\mu}}}

\newcommand{\bXi}{{\boldsymbol{\Xi}}}

\newcommand{\bPi}{{\boldsymbol{\Pi}}}

\newcommand{\rht}{{\tilde{\rho}}}
\newcommand{\rhc}{{\check{\rho}}}

\newcommand{\bSi}{{\boldsymbol{\Sigma}}}

\newcommand{\ups}{\upsilon}
\newcommand{\Ups}{\Upsilon}
\newcommand{\bUp}{{\boldsymbol{\Ups}}}

\newcommand{\bPs}{{\boldsymbol{\Psi}}}

\newcommand{\w}{\omega}
\newcommand{\wh}{{\hat{\omega}}}
\newcommand{\W}{\Omega}



\newcommand{\bzero}{{\mathbf{0}}}
\newcommand{\bone}{{\mathbf{1}}}




==> gww_defs.tex <==
% GWW DEFINITIONS AND ABBREVIATIONS
% Edited by Polina Golland -- Jan 14, 2007



\usepackage{amsthm}
\usepackage{hyperref}
\theoremstyle{definition} 
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\theoremstyle{plain}


% TeX Defs

\usepackage{amsmath} % defines many math commands and
			     % subequations environment, etc  
\usepackage{amssymb}  % get, among others, blackboard bold fonts
                      % defines extra symbols like \gtreqless, etc
\usepackage{verbatim} % get comment environment, + new verbatim 
% \usepackage{amsxtra}  % get, eg, \accentedsymbol

\usepackage{bbm}
\usepackage[mathcal]{euscript}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\boundary}{\p}
\DeclareMathOperator{\cum}{cum}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator*{\lms}{l.i.m.\,}
\DeclareMathOperator{\ev}{\mathbb{E}}
\DeclareMathOperator{\pr}{\mathbb{P}}
\newcommand{\varop}[1]{\var\left[{#1}\right]}
\newcommand{\covop}[2]{\cov\left({#1},{#2}\right)}
\newcommand{\expop}[1]{\exp\left\{{#1}\right\}}
\DeclareMathOperator{\vol}{vol}


\newcommand{\p}{\partial}

% LIST ENVIRONMENTS

\newcounter{actr}
\newenvironment{alist}%
{\begin{list}{(\alph{actr})}{\usecounter{actr}}}{\end{list}}

\newcounter{ictr}
\newenvironment{ilist}%
{\begin{list}{(\roman{ictr})}{\usecounter{ictr}}}{\end{list}}

\iffalse




% SPACING ENVIRONMENTS 

\newenvironment{singlespace}%
{\begin{spacing}{1}}{\end{spacing}}

\newenvironment{onehalfspace}% for 11pt font
{\begin{spacing}{1.21}}{\end{spacing}}

\newenvironment{doublespace}% for 11pt font
{\begin{spacing}{1.62}}{\end{spacing}}

\fi


% THEOREM ENVIRONMENTS


\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corol}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{identity}{Identity}
\newtheorem{defn}{Definition}

\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}

\newtheoremstyle{parant}{}{}{\itshape}{}{\bfseries}{.}{.5em}{#1 \thmnote{(#3)}}
\theoremstyle{parant}
\newtheorem{thmpar}{Theorem}

\theoremstyle{plain}

% \newenvironment{proof}%
% {\noindent{\em Proof: } \begin{singlespace} \small \noindent}%
% {\noindent\qed \end{singlespace}}


\newenvironment{new-proof}[1]%
{ {\em Proof of #1: } \begin{singlespace} \small \noindent}%
{\ \noindent\qed \end{singlespace}}

\newenvironment{new-new-proof}
{ {\em Proof. } \begin{singlespace} \small \noindent}%
{\ \noindent\qed \end{singlespace}}

\newtheorem{quest}{Question}


% Defining Starred sections
\newenvironment{starsec}%
{\renewcommand{\thesection}{\arabic{section}*}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}*}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}*}}%
{\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}}}


\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\card}[1]{\left|#1\right|}
%\newcommand{\comb}[2]{{#1\choose#2}}
\newcommand{\comb}[2]{\binom{#1}{#2}}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\etc}{etc.}
\newcommand{\viz}{viz.}
\newcommand{\etal}{et al.}
\newcommand{\cf}{cf.}


\newcommand{\vect}[3]{\begin{bmatrix} #1 & #2 & \cdots & #3 \end{bmatrix}^\T}

\newcommand{\dsp}{.5\baselineskip}             % double space amount
\newcommand{\down}{\vspace{\dsp}}              % double space command
\newcommand{\ddown}{\vspace{\baselineskip}}    % quadruple space command
\newcommand{\spec}{\hspace*{1pt}}              % little bit of space
\newcommand{\ds}{\displaystyle}                % abbreviation
\newcommand{\ts}{\textstyle}                % abbreviation
\newcommand{\nin}{\noindent}                   % noindent abbreviation
\newcommand{\cvar}[1]{\mathrm{var_{#1}\,}}
% \newcommand{\qed}{\rule[0.1ex]{1.4ex}{1.6ex}}
\newcommand{\mycap}[2]{\caption{\sl #2 \label{#1}}}
\newcommand{\subcap}[1]{{\begin{center}\sl #1\end{center}}}
\newcommand{\ditem}[1]{\item[#1 \hspace*{\fill}]}
\newcommand{\appfig}{\vspace*{1in}\begin{center} Figure appended to
                       end of manuscript. \end{center} \vspace*{1in}}
\newcommand{\psx}[1]{\centerline{\epsfxsize=6in \epsfbox{#1}}}
\newcommand{\psy}[1]{\centerline{\epsfysize=7in \epsfbox{#1}}}
\newcommand{\psxs}[2]{\centerline{\epsfxsize=#1in \epsfbox{#2}}}
\newcommand{\psxsbb}[3]{\centerline{\epsfxsize=#1in \epsfbox[#3]{#2}}}
\newcommand{\psys}[2]{\centerline{\epsfysize=#1in \epsfbox{#2}}}
\newcommand{\convsamp}[3]{\left.\left\{#1 \ast #2\right\}\right|_{#3}}
\newcommand{\gap}{\qquad}
\newcommand{\order}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\arror}[3]{\begin{cases} #1 & #2 \\ 
                                     #3 & \text{otherwise} \end{cases}}
\newcommand{\arrorc}[3]{\begin{cases} #1 & #2 \\ 
                                     #3 & \text{otherwise,} \end{cases}}
\newcommand{\arrorp}[3]{\begin{cases} #1 & #2 \\ 
                                     #3 & \text{otherwise.} \end{cases}}
\newcommand{\darror}[4]{\begin{cases} #1 & #2 \\ #3 & #4 \end{cases}}
% \newcommand{\defeq}{\stackrel{\triangle}{=}}
% \newcommand{\defeq}{\stackrel{\Delta}{=}}
\newcommand{\defeq}{\triangleq}
\newcommand{\pconv}{\stackrel{\mathrm{p}}{\longrightarrow}}
\newcommand{\dconv}{\stackrel{\mathrm{d}}{\longrightarrow}}
\newcommand{\msconv}{\stackrel{\mathrm{m.s.}}{\longrightarrow}}
\newcommand{\pwaeconv}{\stackrel{\mathrm{p.w.a.e.}}{\longrightarrow}}
\newcommand{\peq}{\stackrel{\mathcal{P}}{=}}
% \newcommand{\glt}{ \begin{array}{c} \Hh=H_1 \\ 
%  \renewcommand{\arraystretch}{.3} 
%  \begin{array}{c} > \\ < \end{array}
%  \renewcommand{\arraystretch}{1} \\ \Hh=H_0 \end{array}}

\hyphenation{or-tho-nor-mal}
\hyphenation{wave-let wave-lets}

\newcommand{\crb}{Cram\'{e}r-Rao}  % obsolete
\newcommand{\CR}{Cram\'{e}r-Rao}
\newcommand{\KL}{Karhunen-Lo\`{e}ve}
\newcommand{\sE}{\sqrt{E_0}}
%\newcommand{\pe}{\Prob{\eps}}
\newcommand{\jw}{j\w}
\newcommand{\ejw}{e^{j\w}}
\newcommand{\ejv}{e^{j\nu}}
\newcommand{\wo}{{\w_0}}
\newcommand{\woh}{{\wh_0}}
\newcommand{\sumi}[1]{\sum_{#1=-\infty}^{+\infty}}
\newcommand{\inti}{\int_{-\infty}^{+\infty}}
\newcommand{\intp}{\int_{-\pi}^{\pi}}
\newcommand{\nintp}{\frac{1}{2\pi}\int_{-\pi}^{\pi}}
\newcommand{\inth}{\int_{0}^{\infty}}
%\newcommand{\ev}{\mathbb{E}}
\newcommand{\E}[1]{\ev\left[{#1}\right]}
\newcommand{\Ed}[2]{\ev_{#1}\left[{#2}\right]} % Expectation wrt to distr.
\newcommand{\vard}[2]{\var_{#1}\left({#2}\right)} % Variance wrt to distr.
\newcommand{\bigE}[1]{\ev\bigl[{#1}\bigr]}
\newcommand{\BigE}[1]{\ev\Bigl[{#1}\Bigr]}
\newcommand{\biggE}[1]{\ev\biggl[{#1}\biggr]}
\newcommand{\BiggE}[1]{\ev\Biggl[{#1}\Biggr]}
%\newcommand{\pr}{\mathbb{P}}
\newcommand{\Prob}[1]{\pr\left({#1}\right)}
\newcommand{\prob}[1]{\Prob{#1}}
\newcommand{\Probd}[2]{\pr_{#1}\left[{#2}\right]}
\newcommand{\Pu}[1]{\pr\left[{#1}\right]} % obsolete; same as \Prob now
\newcommand{\Pc}[2]{\pr\left[{#1}\mid{#2}\right]}  % obsolete
\newcommand{\Pcb}[2]{\pr\left[{#1}\Bigm|{#2}\right]} % obsolete
\newcommand{\Q}[1]{Q\left({#1}\right)}
\newcommand{\FT}[1]{\mathcal{F}\left\{{#1}\right\}}
\newcommand{\LT}[1]{\mathcal{L}\left\{{#1}\right\}}
\newcommand{\ZT}[1]{\mathcal{Z}\left\{{#1}\right\}}
%\newcommand{\reals}{\mathbf{R}}
\newcommand{\reals}{\mathbb{R}}
%\newcommand{\ints}{\mathbf{Z}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\compls}{\mathbb{C}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ltwor}{L^2(\reals)}
\newcommand{\ltwoz}{\ell^2(\ints)}
\newcommand{\ltwow}{L^2(\Omega)}
% \newcommand{\ltwo}{\mathbf{L}^2}
% \newcommand{\ltwor}{\mathbf{L}^2 (\reals)}
% \newcommand{\ltwoz}{\mathbf{l}^2 (\ints)}
\newcommand{\sys}[1]{\mathcal{S}\left\{#1\right\}}
\newcommand{\nn}{\nonumber}

\newcommand{\ip}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\di}[2]{d\left({#1},{#2}\right)}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\phase}{\measuredangle}

\newcommand{\Ht}{\mathrm{H}}
\newcommand{\T}{{\mathrm{T}}}
% \newcommand{\R}{\Re\mathit{e}}
% \newcommand{\I}{\Im\mathit{m}}
\DeclareMathOperator{\R}{Re}
\DeclareMathOperator{\I}{Im}

\newcommand{\Eqref}[1]{Eq.~\eqref{#1}}
\newcommand{\exref}[1]{Example~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\corolref}[1]{Corollary~\ref{#1}}
\newcommand{\claimref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}





==> macros/course_header.tex <==
%\pagestyle{myheadings}
%\markright{P. Golland and G. W. Wornell}
\newcommand{\thecoursename}{
Massachusetts Institute of Technology \\
Department of Electrical Engineering and Computer Science

\textsc{6.437 Inference and Information}
}

\newcommand{\theterm}{Spring 2016}
\thispagestyle{empty}



==> macros/defs.tex <==
\newcommand{\courseheader}{
\vspace*{-1in}
\begin{center}
\thecoursename \\
\theterm
\vspace*{0.1in}
\hrule
\end{center}
}

\newcounter{psctr}
\newcounter{probctr}[psctr]
%\renewcommand{\theprobctr}{\arabic{psctr}.\arabic{probctr}}
\newcommand{\problem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr}\nopagebreak

\noindent{#1}

}
\newcommand{\extraproblem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr\ (practice)}\nopagebreak

\noindent{#1}

}

\newcommand{\putfig}[3]{%
\centering
\includegraphics[width=#2]{#1}
\caption{#3}
}

\newcommand{\putfigtwo}[4]{%
\centering
\subfloat[\ ]{\includegraphics[width=#3]{#1}}\\ \vspace*{3ex}
\subfloat[\ ]{\includegraphics[width=#3]{#2}}
\caption{#4}
}

\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif
\DeclareMathAlphabet{\mathbbb}{U}{bbold}{m}{n}  % bb bold numbers
% can also use bbm package, which seems to work w/o pdflatex

%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbb}{bbold}


% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}  
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}

\newcommand{\fxfm}{\stackrel{\mathcal{F}}{\longleftrightarrow}}
\newcommand{\lxfm}{\stackrel{\mathcal{L}}{\longleftrightarrow}}
\newcommand{\zxfm}{\stackrel{\mathcal{Z}}{\longleftrightarrow}}

\DeclareMathOperator*{\gltop}{\gtreqless}
\newcommand{\glt}{\;\gltop^{\Hh=\svH_1}_{\Hh=\svH_0}\;}
\newcommand{\glty}{\;\gltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\gltby}{\;\gltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\DeclareMathOperator*{\geltop}{\genfrac{}{}{0pt}{}{\ge}{<}}
\newcommand{\gelty}{\;\geltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\geltby}{\;\geltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
%\renewcommand{\pe}{\Prob{e}}
\renewcommand{\defeq}{\triangleq}
\newcommand{\like}{\svlike}
\newcommand{\rvlike}{\mathssf{L}}
\newcommand{\sst}{\cl}
\newcommand{\svlike}{L}
\newcommand{\llike}{\rvllike}
\newcommand{\rvllike}{\cl}
\newcommand{\svllike}{l}
\newcommand{\lliket}{\tel}
\newcommand{\bllike}{\rvbllike}
\newcommand{\rvbllike}{\boldsymbol{\cl}}
\newcommand{\svbllike}{\mathbf{l}}
\newcommand{\Qb}{\overline{Q}}
\renewcommand{\comb}[2]{\binom{#1}{#2}}


%% Random/sample variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
% Capitals
\newcommand{\rvA}{{\mathssf{A}}}	% A
\newcommand{\svA}{A}
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\svbA}{{\mathbf{A}}}
\newcommand{\rvFh}{{\hat{\mathssf{F}}}}	% F
\newcommand{\rvF}{{\mathssf{F}}}
\newcommand{\rvHh}{{\hat{\mathssf{H}}}}	% H
\newcommand{\rvH}{{\mathssf{H}}}
\newcommand{\svH}{H}
\newcommand{\svHh}{{\hat{\svH}}}
\newcommand{\rvL}{{\mathssf{L}}}	% L
\newcommand{\svL}{L}
\newcommand{\rvN}{{\mathssf{N}}}	% N
\newcommand{\rvR}{{\mathssf{R}}}	% R
\newcommand{\rvRh}{{\hat{\rvR}}}
\newcommand{\rvS}{{\mathssf{S}}}	% S
\newcommand{\rvSh}{{\hat{\rvS}}}
\newcommand{\rvW}{{\mathssf{W}}}	% W
\newcommand{\rvX}{{\mathssf{X}}}  	% X, random variable
\newcommand{\svX}{X}		  	
\newcommand{\rvXt}{{\tilde{\rvX}}}
\newcommand{\rvY}{{\mathssf{Y}}}	% Y

\newcommand{\rvZ}{{\mathssf{Z}}}	% Z
\newcommand{\rvbZ}{{\mathbsf{Z}}}	
\newcommand{\svZ}{{{Z}}}	
\newcommand{\svbZ}{{\mathbf{Z}}}	

\newcommand{\rva}{{\mathssf{a}}}	% a
\newcommand{\rvah}{{\hat{\rva}}}
\newcommand{\sva}{a}
\newcommand{\svah}{{\hat{\sva}}}
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\svba}{{\mathbf{a}}}
%
\newcommand{\rvb}{{\mathssf{b}}}	% b
\newcommand{\rvbh}{{\hat{\rvb}}}
\newcommand{\svb}{b}
\newcommand{\svbh}{{\hat{\svb}}}
\newcommand{\rvbb}{{\mathbsf{b}}}
\newcommand{\svbb}{{\mathbf{b}}}
%
\newcommand{\rvc}{{\mathssf{c}}}	% c
\newcommand{\rvch}{{\hat{\rvc}}}
\newcommand{\svc}{c}
\newcommand{\svch}{{\hat{\svc}}}
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\svbc}{{\mathbf{c}}}
%
\newcommand{\rvbd}{{\mathbsf{d}}}	% d
\newcommand{\rve}{{\mathssf{e}}}	% e
\newcommand{\sve}{e}
\newcommand{\rvbfe}{{\mathbsf{e}}}
\newcommand{\svbfe}{{\mathbf{e}}}
\newcommand{\rvf}{{\mathssf{f}}}	% f
\newcommand{\svf}{f}
\newcommand{\rvbff}{{\mathbsf{f}}}
\newcommand{\svbff}{{\mathbf{f}}}
\newcommand{\rvg}{{\mathssf{g}}}	% h
\newcommand{\svg}{g}
\newcommand{\rvh}{{\mathssf{h}}}	% h
\newcommand{\rvk}{{\mathssf{k}}}	% k
\newcommand{\svk}{k}
\newcommand{\rvm}{{\mathssf{m}}}	% m
\newcommand{\rvbm}{{\mathbsf{m}}}  
\newcommand{\svm}{{{m}}}
\newcommand{\svbm}{{\mathbf{m}}}
\newcommand{\rvn}{{\mathssf{n}}}	% n
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\rvq}{{\mathssf{q}}}	% q
\newcommand{\svq}{q}
\newcommand{\rvr}{{\mathssf{r}}}	% r
\newcommand{\rvbr}{{\mathbsf{r}}}
\newcommand{\svr}{{r}}
\newcommand{\svbr}{{\mathbf{r}}}
\newcommand{\rvs}{{\mathssf{s}}}	% s
\newcommand{\svs}{s}
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\svbs}{{\mathbf{s}}}
\newcommand{\rvt}{{\mathssf{t}}}	% t
\newcommand{\svt}{t}
\newcommand{\rvbt}{{\mathbsf{t}}}
\newcommand{\svbt}{{\mathbf{t}}}
\newcommand{\rvu}{{\mathssf{u}}}	% u
\newcommand{\svu}{u}
\newcommand{\svuh}{{\hat{\svu}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvv}{{\mathssf{v}}}	% v
\newcommand{\svv}{v}
\newcommand{\svvh}{{\hat{\svv}}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvvh}{{\hat{\rvv}}}
\newcommand{\rvw}{{\mathssf{w}}}	% w
\newcommand{\svw}{w}
\newcommand{\rvwh}{{\hat{\rvw}}}
\newcommand{\svwh}{{\hat{\svw}}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvx}{{\mathssf{x}}}	% x, random variable
\newcommand{\rvxh}{{\hat{\rvx}}}
\newcommand{\rvxt}{{\tilde{\rvx}}}
\newcommand{\svx}{x}			% sample value
\newcommand{\svxh}{{\hat{\svx}}}
\newcommand{\svxt}{{\tilde{\svx}}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvbxh}{{\hat{\rvbx}}}
\newcommand{\rvbxt}{{\tilde{\rvbx}}}
\newcommand{\svbx}{{\mathbf{\svx}}}
\newcommand{\svbxt}{{\tilde{\svbx}}}
\newcommand{\svbxh}{{\hat{\mathbf{x}}}}
\newcommand{\rvy}{{\mathssf{y}}}	% y
\newcommand{\rvyh}{{\hat{\mathssf{y}}}}
\newcommand{\svy}{y}
\newcommand{\rvyt}{{\tilde{\rvy}}}
\newcommand{\svyt}{{\tilde{\svy}}}
\newcommand{\svyh}{{\hat{\svy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvbyt}{{\tilde{\rvby}}}
\newcommand{\svby}{{\mathbf{y}}}
\newcommand{\svbyt}{{\tilde{\svby}}}
\newcommand{\rvz}{{\mathssf{z}}}	% z
\newcommand{\rvzh}{{\hat{\rvz}}}
\newcommand{\rvzt}{{\tilde{\rvz}}}
\newcommand{\svz}{z}
\newcommand{\svzh}{{\hat{\svz}}}
\newcommand{\rvbz}{{\mathbsf{z}}}
\newcommand{\svbz}{{\mathbf{z}}}

% Handle uppercase Greek differently
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\svTh}{\Theta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\svbTh}{\boldsymbol{\Theta}}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\svPh}{\Phi}
\newcommand{\rvbPh}{\bsfPhi}
\newcommand{\svbPh}{\boldsymbol{\Phi}}

\newcommand{\ddx}{\frac{\diff}{\diff \svx}}
\newcommand{\ddbx}{\frac{\diff}{\diff\svbx}}
\newcommand{\ppx}{\frac{\p}{\p \svx}}
\newcommand{\ppbx}{\frac{\p}{\p\svbx}}
\newcommand{\ddy}{\frac{\diff}{\diff \svy}}
\newcommand{\ddby}{\frac{\diff}{\diff\svby}}
\newcommand{\ppy}{\frac{\p}{\p \svy}}
\newcommand{\ppby}{\frac{\p}{\p\svby}}

\def\setTh{\text{$\mksetTh$}}  % make caligraphic Theta
\def\mksetTh{\setbox0\hbox{$\mathcal{O}$}%
    \rlap{\hbox to \wd0{\hss\raisebox{.2ex}{\hspace*{.07em}\textbf{-}}\hss}}\box0}

%  --add new macros below this line--

\newcommand\indep{\protect\mathpalette{\protect\indepT}{\perp}}
\def\indepT#1#2{\mathrel{\rlap{$#1#2$}\mkern3mu{#1#2}}}
\newcommand{\truex}{\svx}
\newcommand{\obsy}{\svy}
\newcommand{\dummyx}{a}
\newcommand{\dummybx}{\ba}
\newcommand{\dummyy}{b}
\newcommand{\dummyby}{\bb}
\newcommand{\dummyz}{c}
\newcommand{\Db}{D_\mathrm{B}}   % binary divergence
\newcommand{\Hb}{H_\mathrm{B}}   % binary entropy
\newcommand{\Hhb}{\Hh_\mathrm{B}} % Bayes decision rule
\newcommand{\Hhnp}{\Hh_\mathrm{NP}} % Neyman-Pearson decision rule
\newcommand{\Hhm}{\Hh_\mathrm{M}} % minimax decision rule
\newcommand{\alphA}{\cA}
\newcommand{\alphB}{\cB}
\newcommand{\alphE}{\cE}
\newcommand{\alphL}{\cL}
\newcommand{\alphV}{\cV}
\newcommand{\cardV}{M}
\newcommand{\alphR}{\cR}
\newcommand{\alphS}{\cS}
\newcommand{\alphT}{\cT}
\newcommand{\alphU}{\cU}
\newcommand{\alphW}{\cW}
\newcommand{\alphX}{\cX}
\newcommand{\cardX}{L}
\newcommand{\alphY}{\cY}
\newcommand{\alphZ}{\cZ}
\newcommand{\cardY}{M}
\newcommand{\efdim}{K}
\newcommand{\dimX}{K}
\newcommand{\dimY}{N}
\newcommand{\alphH}{\cH}

\newcommand{\sumX}{\sum_{\svx\in\alphX}}
\newcommand{\sumY}{\sum_{\svy\in\alphY}}

\newcommand{\fisher}{J}
\newcommand{\Fisher}{\bJ}
\newcommand{\bfisher}{\bJ}
\newcommand{\score}{S}
\newcommand{\Score}{\bS}
\newcommand{\bscore}{\bS}
\newcommand{\objfn}{\varphi}
\newcommand{\varobjfn}{\tilde{\objfn}}




\renewcommand{\emptyset}{\varnothing}
\renewcommand{\approx}{\cong}

% functional dot

\def\fndot{\, \cdot \,}

% exponential

\newcommand{\eexp}[1]{e^{#1}}

% iid

\newcommand{\iid}{i.i.d.}

% convergence

\newcommand{\convp}{\stackrel{\mathrm{p}}{\longrightarrow}}
\newcommand{\convas}{\stackrel{\mathrm{a.s.}}{\longrightarrow}}
\newcommand{\convwpone}{\convas}
\newcommand{\convd}{\stackrel{\mathrm{d}}{\longrightarrow}}
\newcommand{\convD}{\stackrel{\mathrm{D}}{\longrightarrow}}

% stochastic approximation

\newcommand{\pun}{p_\circ}
\newcommand{\punh}{\hat{p}_\circ}
\newcommand{\qun}{q_\circ}
\newcommand{\qunh}{\hat{q}_\circ}

\newcommand{\genf}{f}
\newcommand{\genfb}{\bar{f}}
\newcommand{\genfbh}{\hat{\bar{\rvf}}}


\DeclareMathOperator{\neb}{ne}
\newcommand{\bep}{{\boldsymbol{\varepsilon}}}

\newcommand{\gauss}{\mathtt{N}}
\newcommand{\bern}{\mathtt{B}}
\newcommand{\unif}{\mathtt{U}}
\newcommand{\poiss}{\mathtt{P}}
\newcommand{\betad}{\mathtt{Beta}}
\newcommand{\gammad}{\mathtt{Gamma}}
\newcommand{\expd}{\mathtt{E}}
\newcommand{\expfam}{\mathcal{E}}

\newcommand{\kron}{\mathbbb{1}}
%\newcommand{\kron}{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}
%\DeclareMathOperator{\kron}{\leavevmode\hbox{\small\rm1\normalsize\kern-.33em1}}

\newcommand{\dotleq}{\stackrel{.}{\leq}}
\newcommand{\dotlt}{\stackrel{.}{<}}
\newcommand{\dotgeq}{\stackrel{.}{\geq}}
\newcommand{\dotgt}{\stackrel{.}{>}}
\newcommand{\Ps}[1]{P\left\{#1\right\}}
\newcommand{\Qs}[1]{Q\left\{#1\right\}}

\newcommand{\diff}{\mathrm{d}}

% from 6.008

\newcommand{\sd}{p_\rvx}  % steady-state distribution
\newcommand{\td}{W}    % transition distribution
\newcommand{\sdv}{\bp_\rvx}  % steady-state distribution vector
\newcommand{\tdm}{\bW}  % transition distribution matrix
\newcommand{\tde}{w}    % transition distribution matrix elements
\newcommand{\sde}{p}    % steady-state distribution vector elements
\newcommand{\bigO}{\mathcal{O}}



==> macros/gww_theorems.tex <==
% GWW DEFINITIONS AND ABBREVIATIONS
% Edited by Polina Golland -- Jan 14, 2007



\usepackage{amsthm}


\theoremstyle{definition} 
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\theoremstyle{plain}


% THEOREM ENVIRONMENTS


\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corol}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{fact}{Fact}
\newtheorem{identity}{Identity}
\newtheorem{defn}{Definition}

\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}

\newtheoremstyle{parant}{}{}{\itshape}{}{\bfseries}{.}{.5em}{#1 \thmnote{(#3)}}
\theoremstyle{parant}
\newtheorem{thmpar}{Theorem}

\theoremstyle{plain}

% \newenvironment{proof}%
% {\noindent{\em Proof: } \begin{singlespace} \small \noindent}%
% {\noindent\qed \end{singlespace}}


\newenvironment{new-proof}[1]%
{ {\em Proof of #1: } \begin{singlespace} \small \noindent}%
{\ \noindent\qed \end{singlespace}}

\newenvironment{new-new-proof}
{ {\em Proof. } \begin{singlespace} \small \noindent}%
{\ \noindent\qed \end{singlespace}}

\newtheorem{quest}{Question}


% Defining Starred sections
\newenvironment{starsec}%
{\renewcommand{\thesection}{\arabic{section}*}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}*}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}*}}%
{\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}}}


